MapCoder: Multi-Agent Code Generation for Competitive Problem Solving

Code synthesis, which requires a deep understanding of complex natural language problem descriptions, generation of code instructions for complex algorithms and data structures, and the successful execution of comprehensive unit tests, presents a significant challenge. While large language models (LLMs) demonstrate impressive proficiency in natural language processing, their performance in code generation tasks remains limited. In this paper, we introduce a new approach to code generation tasks leveraging multi-agent prompting that uniquely replicates the full cycle of program synthesis as observed in human developers. Our framework, MapCoder, consists of four LLM agents specifically designed to emulate the stages of this cycle: recalling relevant examples, planning, code generation, and debugging. After conducting thorough experiments, with multiple LLM ablations and analyses across eight challenging competitive problem-solving and program synthesis benchmarks, MapCoder showcases remarkable code generation capabilities, achieving new state-of-the-art results (pass@1) on HumanEval (93.9%), MBPP (83.1%), APPS (22.0%), CodeContests (28.5%), and xCodeEval (45.3%). Moreover, our method consistently delivers superior performance across various programming languages and varying problem difficulties. We open-source our framework at https://github.com/Md-Ashraful-Pramanik/MapCoder.

==> sections/old/experimental-setup-old.tex <==
\section{Experimental Setup}
% \eunus{give an overview what's coming next...like We first present seven benchmark datasets:..., and then discuss the baselines we used...., and present the evaluation metrics}

In this section, we  first present seven benchmark datasets, the competitive methods, and the evaluation metrics used in our experiments.

\subsection{Benchmark Datasets}
%We assessed the effectiveness of our proposed prompting method across seven benchmark datasets, each offering a distinct set of challenges. These datasets are detailed below:
We have evaluated the competitive approaches using seven benchmark datasets, each offering a distinct set of challenges. The details of these datasets are summarized as follows.
% \eunus{dont need subsubsection...just use bolface on the first appearance??}
%\subsubsection{HumanEval}
\textbf{HumanEval} \cite{chen2021codex}, introduced by OpenAI, comprises 164 handwritten programming problems. %Each problem includes a problem description and its corresponding function signature. 
This dataset is known for featuring relatively easy problems, serving as a foundational benchmark for evaluating language models in code generation task.

%\subsubsection{HumanEval-ET} 
\textbf{HumanEval-ET} \cite{dong2023codescore} stands as an extension of the HumanEval dataset. While it retains the problems from HumanEval, its test set incorporates over 100 additional tests. These additional tests encompass corner cases, providing a more comprehensive evaluation to ensure the correctness of a solution.

%\subsubsection{MBPP} 
\textbf{The Mostly Basic Programming Problems (MBPP)} \cite{austin2021program} dataset comprises 974 short Python programs generated through crowd-sourcing. For a fair comparison with the competitive methods, we have used a subset of this dataset, consisting of 397 problems with function signatures, which was previously used in Reflexion \cite{shinn2023reflexion}. As the dataset does not contain sample IOs, we generate one sample IO for each problem from the available test cases. For fair comparison we have eliminated that test case for other approaches. 
\ashraful{Vaia please address this.}
%This dataset does not contain any sample IO. For this reason we have taken one test case from the private test set as sample IO.

%\subsubsection{MBPP-ET} 
\textbf{MBPP-ET} \cite{dong2023codescore} is an extension of the MBPP dataset, which provides additional challenges to assess the robustness of language models in handling diverse scenarios. 
% Both MBPP and MBPP-ET do not contain sample test cases. For this reason, we have taken one test case from an extended test set that is not in the normal test set as a representative of the sample test case. While final evaluation on MBPP-ET we have eliminated that test case for fair comparison among all other approaches. 
% \ashraful {rizwan vaia please correct it if there is some misunderstanding}

%\subsubsection{APPS}
\textbf{The Automated Programming Progress Standard (APPS)} \cite{hendrycks2021measuring}, comprises a collection of programming problems sourced from diverse open-access coding platforms, including Codeforces and Kattis. These problems span a wide spectrum of difficulty levels, ranging from introductory challenges to those encountered in collegiate-level competitions. In total, the APPS dataset encompasses 10,000 coding problems, featuring a comprehensive set of 131,777 test cases designed for validating solutions. For our evaluation, we adopt a random sampling strategy to select 150 problems, where 50 with introductory-level difficulty, 52  with  interview-level challenges, and  48 with competition-level complexity.

%For this work, we conducted a random sampling of 150 problems from the APPS dataset. This sample is strategically composed, with 50 problems representing introductory difficulty levels, another 52 representing interview-level challenges, and a final set of 48 capturing problems characteristic of competition-level complexity. This diverse subset enables us to assess the effectiveness of our proposed prompting method across various difficulty scenarios, offering insights into its performance across a spectrum of real-world coding challenges.

%\subsubsection{xCodeEval}
\textbf{xCodeEval} \cite{khan2023xcodeeval} stands as the most extensive executable multilingual multitask benchmark, comprising a vast collection of 25 million document-level coding examples that span up to 17 programming languages. In our study, we take the validation set of this benchmark, which includes 106 problems. %The problems within the validation set served as the basis for our evaluation, allowing us to assess the performance of our proposed prompting method within the context of these diverse coding challenges.

%\subsubsection{CodeContest}
\textbf{CodeContests} \cite{li2022competition} is a dataset focused on competitive programming, encompassing a compilation of programming problems drawn from diverse sources. The dataset comprises approximately 3,760 problems in its training set, 117 problems in the validation set, and 165 problems in the test set. We use 165 test set problems from this dataset in our experiments. %For our study, we specifically utilized the test set, leveraging its 165 problems to assess and evaluate the performance of our proposed prompting method in the context of competitive programming challenges.


\subsection{Competitive Approaches}
We have evaluated our proposed approach, \tool, and compared the results with several baselines and state-of-the-art (SoTA) approaches. 

% \eunus{not all methods are based on prompting, right? some are dedicated models for code generation...?? os the following can be merged with baselines..also we should write about MapCoder (specifically which background model you used..)} 
% We evaluated different prompting approaches using ChatGPT (gpt-3.5-turbo-1106) and GPT-4 (gpt-4-1106-preview) from OpenAI, and Gemini Pro from Google.  %\cite{achiam2023gpt}

%\subsection{Baselines}

\textbf{Direct Prompting} involves instructing the Language Models (LLMs) to generate code in a zero-shot setting, where no examples or additional information are provided. Leveraging the extensive training data of modern LLMs, this approach relies on the model's inherent capabilities to solve programming problems without explicit guidance.

\textbf{Chain of Thought Prompting} first introduced in \cite{wei2022chain}. It directs the model to address a problem incrementally, breaking it down into step-by-step solutions rather than solving it as a whole. This method incorporates intermediate reasoning steps, enabling LLMs to effectively tackle complex problems. Few-shot prompting can further enhance its performance. By randomly selecting example problems and generating their step-by-step solutions, we created few-shot examples.

\textbf{Self-Planning Prompting}, as proposed in \cite{jiang2023self}, divides the code generation task into two distinct stages: the Planning phase and the Implementation phase. In the Planning phase, a plan to solve the given problem is generated before passing it to the LLM for execution. Few-shot prompting is employed in the plan generation phase to provide the LLM with relevant examples for improved planning. We utilized examples from the original paper for the HumanEval dataset and randomly selected examples from other datasets, aligning with the principles outlined in the Self-Planning Prompting approach.

\textbf{Analogical Reasoning Prompting}, as introduced by \cite{yasunaga2023large}, presents another innovative approach to prompting Language Models (LLMs) for programming tasks. In this method, the LLMs are guided to first generate relevant exemplars of a programming problem and subsequently solve the original problem using the insights gained from these examples. By explicitly instructing LLMs to recall relevant problems from their extensive training data, Analogical Reasoning Prompting capitalizes on the model's ability to remember and apply solutions to similar problems. 

\textbf{Reflexion} proposed in \cite{shinn2023reflexion}, employs a unique approach to learning from past mistakes through verbal reinforcement. In this methodology, Reflexion generates unit tests based on the problem description and utilizes these test cases to evaluate the proposed solution. If the solution fails in the generated unit tests, Reflexion provides constructive verbal feedback to the model, guiding it to enhance the solution. Conversely, when the solution successfully passes the generated unit tests, it is then considered for final evaluation. 
% This iterative process of generating tests, evaluating solutions, and providing verbal feedback aims to enhance the model's performance through reinforcement.

\textbf{AlphaCodium} approach, as put forth by \cite{ridnik2024code}, introduces a novel strategy for tackling programming problems. The method involves iteratively generating code and subsequently refining it based on input-output tests. In addition to the public test cases, AlphaCodium generates additional test cases to enhance the diversity of the evaluation process. After code generation, the approach involves an iterative fixing process, where the generated code is refined and improved based on the feedback obtained from the input-output tests. 

We have evaluated these prompting approaches using ChatGPT (gpt-3.5-turbo-1106) and GPT-4 \cite{achiam2023gpt} (gpt-4-1106-preview) from OpenAI, and Gemini Pro \cite{geminiteam2023gemini} from Google. 

% We have used another 
% \textbf{MoTCoder} The Modular-of-Thought Coder (MoTCoder) model, introduced by \cite{li2023motcoder}, presents an innovative approach to solve a programming problem through a fine-tuned Large Language Model (LLM). MoTCoder adopts a modular approach, breaking down the problem-solving process into distinct steps. In the initial phase, the model generates the necessary sub-modules, which include function headers and docstrings essential for solving the given problem. Subsequently, MoTCoder implements these modules in the next step. Finally, it combines these individually generated and implemented modules to derive a comprehensive and final solution to the programming problem. This modular strategy enhances the model's ability to systematically approach complex problem-solving tasks.


% \subsubsection{Implementation Details of the Baselines}
% In most of the cases we have used the code proposed by the corresponding model for our experiments. 
\subsection{Evaluation Metric}
We employed the Pass@k evaluation metric, where $k$ denotes the number of solutions to be generated. If at least one of the solutions is correct, the model is deemed successful for that problem. Pass@k represents the fraction of problems for which the model succeeded according to this criterion.


==> sections/old/intro-old.tex <==
\section{Introduction}
\label{sec:intro}
Computer Programming has emerged as an ubiquitous problem-solving tool that brings tremendous benefits to every aspects of our life \cite{li2022competition, parvez-etal-2018-building, knuth1992literate}. To maximize programmers’ productivity, and enhance accessibility, automation in program synthesis is paramount. W/ the growth of LLMs, significant advancements have been made in program synthesis—driving us in an era where we can generate fully executable code, requiring no human intervention~\cite{chowdhery2022palm, nijkamp2022codegen}.

However, despite LLMs' initial success and the scaling up of model size and data, many of these models  still struggle to perform well on complex problem-solving tasks specially in competitive programming problems \cite{austin2021program}. To mitigate this gap, in this paper, we introduce {\bf \toolnospace}: a {\bf M}ulti-{\bf A}gent {\bf P}rompting Based Code Generation approach that can seamlessly synthesize solutions for competition-level programming problems. 

{Competitive programming} or {competition-level code generation}, often regarded as the pinnacle of problem-solving, is an extremely challenging task. It requires a deep comprehension of NL problem descriptions, multi-step complex reasoning beyond mere memorization, excellence in  algorithms and data structures, and the capability to generate substantial code that produces desired outputs aligned with comprehensive test cases \cite{khan2023xcodeeval}. 

% Computer programming plays a vital role in modern problem-solving, offering extensive benefits across various domains \cite{li2022competition, parvez-etal-2018-building, knuth1992literate}. With the rise of Large Language Models (LLMs), significant progress has been made in automating program synthesis, leading to the ability to generate fully executable code without human intervention \cite{chowdhery2022palm, nijkamp2022codegen}. Despite these advancements, LLMs often struggle with complex problem-solving tasks, particularly in competitive programming scenarios. These challenges highlight the need for innovative approaches to bridge this gap. In response, this paper introduces \tool, a \textbf{M}ulti-\textbf{A}gent \textbf{P}rompting Based Code Generation approach designed to synthesize solutions for competition-level programming problems. 

% Competitive programming, known for its complexity and rigor, requires advanced problem-solving skills beyond simple memorization. It demands intricate reasoning, algorithmic expertise, and the ability to generate precise code aligned with comprehensive test cases \cite{khan2023xcodeeval}. 


\begin{figure*}
    \centering
    \includegraphics[width=0.99\textwidth]{figures/MapCoder.pdf}
    % \caption{Overview of \ourapproach. \tool is structured around four distinct agents: the Self-Retrieval Agent, Planning Agent, Coding Agent, and Debugging Agent. Initially, the Self-Retrieval Agent retrieves relevant examples (step-1) related to the given problem. These examples are then passed to the Planning Agent, which generates a plan with a certain level of confidence (step-2). Subsequently, the plan with the highest confidence is handed over to the Coding Agent for code generation (step-3). After generating the code, we test it using sample IO, and in case of failure, we give the code to a debugging agent for debugging (step-4).The Debugging Agent tries to fix the bugs of the generated code. Debugging agent may try several times (step-5 and 6). If the Debugging Agent fails to rectify any errors, it goes to the planning agent again (step-7). The process then iterates by considering the next plan with the next highest confidence level (step-8). This iterative process continues until either a successful solution is obtained or all plans have been explored. The numbers enclosed within small yellow circles denote the steps involved in this process.}
    \vspace{-5mm}
    \caption{
    % \vspace{-1mm}
    Overview of \tool (top). 
    % This schematic illustrates the orchestrated workflow of \toolnospace, comprising four agents: (Self) Retrieval, Planning, Coding, and Debugging. 
    It starts with a retrieval agent that generates relevant examples itself, followed by planning, coding, \& iterative debugging agents. Our dynamic traversal (bottom) considers the confidence of the generated plans as their reward/utility scores \& leverage them to guide the code generation accordingly.}
    \label{fig:map-coder-overview}
    \vspace{-2mm}
\end{figure*}  

Early approaches utilizing LLMs for code generation employ a direct prompting approach, where LLMs generate code directly from problem descriptions and sample I/O \cite{chen2021codex}. Recent methods like chain-of-thought \citep{CoT} advocate modular or pseudo code-based generation to enhance planning and reduce errors, while retrieval-based approaches such as  \citet{parvez2021retrieval} leverage relevant problems \& solutions to guide LLMs' code generations. However, gains in such approaches remains limited in such a complex task like code generation where LLMs' generated code often fails to pass the test cases and they do not feature bug-fixing scheme \cite{ridnik2024code}. 

% A promising solution to this challenge is self-reflection, which iteratively evaluates the generated code against test cases, self-reflects on mistakes and modifies accordingly \cite{shinn2023reflexion, chen2022codet}. However, such approaches may be sub-optimal. Firstly \eunus{do we have any other limitation?}, during code generation, they only leverage the problems description itself in a 0-shot manner,  whereas previous studies indicate that superior problem-solving capabilities are attained when using in-context exemplars \citep{shum-etal-2023-automatic, zhang2022automatic, CoT}.


% A promising solution to this challenge is self-reflection, which iteratively evaluates the generated code against test cases, reflects on mistakes, and modifies accordingly \cite{shinn2023reflexion, chen2022codet}. However, such approaches has limitations too. Firstly, while previous studies indicate that superior problem-solving capabilities are attained when using in-context exemplars \citep{shum-etal-2023-automatic, zhang2022automatic, CoT}, such approaches, during code generation, only leverage the problem description itself in a 0-shot manner. Consequently, their gains can be limited.

A promising solution to this challenge is self-reflection, which iteratively evaluates the generated code against test cases, reflects on mistakes, and modifies accordingly \cite{shinn2023reflexion, chen2022codet}. However, such approaches have limitations too. Firstly, while previous studies indicate that superior problem-solving capabilities are attained when using in-context exemplars \citep{shum-etal-2023-automatic, zhang2022automatic, CoT}, these approaches, during code generation, only leverage the problem description itself in a 0-shot manner. Consequently, their gains can be limited.

% fail to harness additional learning signals, such as the previously mentioned prompt augmentation through retrieval. Studies indicate that superior problem-solving capabilities are attained when using in-context exemplars \citep{shum-etal-2023-automatic, zhang2022automatic, CoT}.

% To tackle this challenge, we develop \tool by drawing inspiration from real programmers' thought process. The human problem-solving cycle involves recalling past solutions, sketching a plan, writing code, and debugging. \tool imitates these steps using LLM agents - retrieval, planning, coding, and debugging. In contrast to relying on external code retrieval models, we empower the LLM agent to autonomously retrieve relevant problems itself \cite{yasunaga2023large}. Additionally, we design a new structured pipeline schema that cascades LLM agents intelligently, and a dynamic iteration protocol for traversing through our agents to enhance the generation procedure leveraging the agents. Figure \ref{fig:map-coder-overview} shows an overview of our approach, \tool.

To confront the above challenge, we develop \tool augmenting the generation procedure w/ possible auxiliary supervisions.  We draw inspiration from the cognitive processes of real programmers and their adept utilization of various learning signals throughout the procedure. The human problem-solving cycle involves recalling past solutions, planning, code writing, and debugging. \tool imitates these steps using LLM agents - retrieval, planning, coding, and debugging. In contrast to relying on human annotated examples, or external code retrieval models,  we empower our retrieval agent to autonomously retrieve relevant problems itself \cite{yasunaga2023large}.
Moreover, we design a novel structured pipeline scheme that intelligently cascades the LLM agents and incorporates a dynamic iteration protocol to enhance the generation procedure at every step. Figure \ref{fig:map-coder-overview} shows an overview of our approach, \tool.

Additionally, existing self-reflection methods relies on extra test cases generated by LLM agents or external tools, compounding the challenges. Test case generation is equally challenging as code generation \cite{pacheco2007feedback}, with success reliant on the model and the dataset. Incorrect test cases can lead to erroneous code. Blindly editing code based on these test cases can undermine problem-solving capabilities. For instance, while self-reflection boosts GPT-4's performance on the HumanEval dataset, it drops by 3\% on the MBPP dataset \cite{shinn2023reflexion}. Upon identification, to validate this, on the HumanEval dataset itself, we replace their GPT-4 with ChatGPT, and see that model performance drops by 26.3\%. Therefore, our debugging agent performs unit tests and bug fixing using only the sample I/O, w/o any artifact-more plausible for real-world widespread adoption. 

We evaluate \tool on seven popular programming synthesis benchmarks including both basic programming like HumanEval, MBPP and challenging competitive program-solving benchmarks like APPS, CodeContests and xCodeEval. With multiple different LLMs including ChatGPT, GPT-4, and Gemini Pro, our approach significantly enhances their problem-solving capabilities - consistently achieving new SOTA performances, outperforming strong baselines like Reflexion \citep{shinn2023reflexion}, and AlphaCodium \citep{ridnik2024code}. Moreover, our method consistently delivers superior performance across various programming languages \& varying problem difficulties. Furthermore, with detailed ablation studies, we analyze \tool to provide more insights. 

% Our contributions encompass: 
% \begin{itemize}
%     \item please write from my intro.
% \end{itemize}

\iffalse
{
% Subsequent works can be summarized in three categories. (i) Recall, (ii) Chain/plan  (iii) gen (iv) test/debug




Furthermore, we propose to leverage the code. 


% \ashraful{updated based on your comments}

% The emergence of Large Language Models (LLMs) has revolutionized Natural Language Processing (NLP), with remarkable success observed across various domains\eunus{cite..}. One such domain experiencing significant advancements is sequence-to-code generation. In contrast to typical sequence-to-sequence tasks, where sentences can be expressed diversely without changing their meaning, code generation demands strict adherence to precise syntax for producing executable code.
% This complexity underscores the intricacy of code generation tasks compared to traditional NLP tasks. \eunus{i dont think the following sentences are important...rather thn we should first define the problem (input-ouput, and then talk about the importance of this task and the challenges that we are facing.. and then in the following para should discuss different groups of tasks ans their limitations...} Recent progress in code generation has shifted focus from evaluating similarity metrics like CodeBLEU\footnote{CodeBLEU measures the similarity between generated code and reference code} to executing generated code with test cases, indicating a move towards LLMs emulating professional coding proficiency \eunus{why do we need to say this as this is only for evaluation..}. While LLMs still face challenges in competitive programming, diverse prompting approaches are steadily enhancing code generation performance\eunus{suddenly you are talking about competitive programming}.

\eunus{i cannot get why tihs para is here....it seems out of blow...it should come much later as your intuition not the fact..}
Understanding how a human evolves into an expert coder provides valuable insights. Mastery begins with extensive practice to memorize programming language syntax, followed by learning traditional problem-solving algorithms such as brute-force, greedy, divide-and-conquer, dynamic programming, recursion, and more. Upon mastering programming basics, an expert coder approaches new problems by recalling similar ones and applying analogous solutions. Before commencing coding, a well-defined plan is conceptualized either mentally or on paper. Subsequently, the coder generates code, test it with sample test cases, and rectifies any bugs until it passes all the test cases. \eunus{is there any reference that these are the fixed set of steps??} This process can be divided into six key steps: 1) Recalling exemplars, 2) Planning, 3) Code generation, 4) Generation of additional test cases, 5) Testing, and 6) Debugging.

We can broadly divide the existing works on code generation tasks\eunus{have we said before that sequence-to-code is referred as code generation tasks} into three  categories\eunus{can we generalize the category without relating to the above steps...}: i) example retrieval (step 1 and 3) \cite{yasunaga2023large}, 2) planning generation (step 2 and 3) \cite{jiang2023self}, 3) additional test case generation and iterative code updating based on test reports (step 3 to 6) \cite{shinn2023reflexion, chen2022codet, le2022coderl}. As per best of our knowledge we can not find any work that consists of all the above steps. Moreover, the accuracy of additional test case generation poses challenges, depending on dataset type, LLM capability, and programming language nuances.  \cite{chen2022codet}. Even the LLM may be trained with dataset like HumanEval \cite{chen2021codex} thus resulting in data leakage. For example Reflexion \cite{shinn2023reflexion} performs well in HumanEval \cite{chen2021codex} but failed to improve performance in MBBP \cite{austin2021program} dataset. Reflexion also skip the additional test case generation part for competitive programming problems. We have also observed that the performance dropped if we switch the from GPT4 to ChatGPT. Our method for Code Generation bridges the gap between human problem-solving approaches and state-of-the-art methods by proposing a multi-agent prompting approach where all these steps are being considered and prompted through different agents.

Motivated by the sequential workflow of an expert programmer, we present a novel prompting approach named \textbf{M}ulti-\textbf{a}gent \textbf{p}rompting for code generation (\ourapproach). \tool has four key agents: 1) A Retrieval agent for retrieving the exemplars, 2) a Planner for plan generation, 3) a Coder for code synthesis, and 4) a Debugging agent for comprehensive testing and bug fixing. Notably, our Retrieval phase employs self-retrieval, eliminating the need for human assistance in the first agent. Due to the complexity involved in accurately creating additional test cases for complex problems, our approach omits the generation of additional test cases. Because if one wrong test case is generated that will results in wrong code. The generation of test cases from problem descriptions represents a distinct research problem, and excluding this step in \tool aligns with current limitations in the field. Leveraging \ourapproach, we conducted extensive experiments on both simple and competitive-level problem sets, showcasing its superior performance compared to existing methods across a variety of code generation benchmarks. Figure \ref{fig:map-coder-overview} demonstrates the overview of \tool .





\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/MapCoder.pdf}
    \caption{Overview of \ourapproach.}
    \label{fig:map-coder-overview}
\end{figure*}  

\eunus{not readabale..let's discuss..also describe this process clearly}
\ashraful{updated. see Figure\ref{fig:map-coder-overview}}
    

\eunus{you use very weak verbs and seem you dont have any contribution...look at other similar papers and write in more active and strong verb....we develop...we evaluate...}
\ashraful{updated}

Our contributions encompass: 
\begin{itemize}
    \item We breach the gap in code generation task by providing a prompting approach that combines all the steps like a human coder. 
    \item We develop a novel prompting approach \tool for generating code from text in any programming language.\tool can handle both straightforward and competitive-level programming challenges.
    \item We evaluate \tool in various code generation benchmarks and achieve state-of-the-art performance across various code generation benchmarks.
\end{itemize}
\fi




==> sections/old/our-approach.tex <==
\section{\tool}
\label{sec:mapcoder}
Our goal is to develop a multi-agent code generation approach for competitive problem-solving. In order to do so, our framework, \toolnospace, replicates the human programming cycle through four LLM agents - retrieval, plan, code, debug. We devise a pipeline sequence for \toolnospace, intelligently cascading the agents in a structured way and enhancing each agent's capability by augmenting in-context learning signals from previous agents in the pipeline. However, not all the agent responses/outputs are equally useful. Therefore, additionally, \tool features an adaptive agent traversal scheme to interact among corresponding agents dynamically, iteratively enhancing the generated code by, for example, fixing bugs, while maximizing the usage of the LLM agents.  In this section, we first discuss the agents as per the pipeline, their prompts, and interactions, followed by the dynamic agent traversal protocol in \tool towards code generation for competitive problem-solving. 

\subsection{Retrieval Agent}
\label{subsec:our-algo-agent-1}
Our first agent, the \emph{Retrieval Agent}, recalls past relevant problem-solving instances, akin to human memory. It finds (user-defined) $k$ similar problems without manual crafting or external retrieval models. Instead, we leverage the LLM agent itself, instructing it to generate such problems. Our prompt extends the analogical prompting principles \cite{yasunaga2023large}, generating examples and their solutions simultaneously, along with additional metadata (e.g., problem description, code, \& plan) to provide to the following agents as auxiliary data.
We adopt a specific sequence of instructions, crucial for the prompt's effectiveness. Initially, we instruct the LLM to produce both similar and distinct problems along with their solutions, facilitating problem planning reverse-engineering. Then, for our \emph{Planning Agent}, we prompt LLMs to generate solution code step-by-step, allowing post-processing to form the corresponding plan. Finally, we direct the LLM to generate relevant algorithms and provide instructional tutorials, enabling the agent to reflect on underlying algorithms and generate algorithmically similar examples.
% Our first agent in the pipeline is a \emph{Retrieval Agent}. Similar to humans' recalling of past relevant problem-solving, our retrieval agent also finds (user-defined) $k$ similar problems. Instead of manually crafting the similar examples or using external retrieval models, we leverage the LLM agent itself as a proxy and instruct it to generate such problems.  Our prompt for self-retrieval agent is built upon the analogical prompting \cite{yasunaga2023large} which is a single-agent approach, generating only the example and the final solution, at the same time. In our prompt, we also instruct the agent to provide additional metadata for the examples (e.g., problem description, code, \& plan) to provide to the following agents as auxiliary data.  Appendix Figure \ref{fig:prompt-agent-1} shows the prompt.  Note that we adopt a specific sequence of instructions in the prompt which is a crucial design choice. Our prompt first asks the LLM to produce both similar and distinct problems along with their solutions, enabling it to reverse-engineer the problem planning from the generated content. In order to do so, inside the prompts for our \emph{Planning Agent}, we ask  the LLMs to generate the solution code as per the chain-of-thought method (step-by-step) so that we can post-process the outputs and combine the steps as the corresponding plan for the example code.
% We then direct the LLM to generate relevant algorithms for the given problem and provide instructional tutorials to enable the agent reflecting on the underlying algorithms and  generate examples that are algorithmically close too.   
% \rizwan{Ashraful, I don't get this. In the example code generation, u apply CoT, then from that backtrack to plan, plan is CoT are different?  }


% \begin{itemize}
%     \itemsep0em
%     \small 
%     \item First, we prompt the LLM to produce both similar and distinct problems along with their solutions, enabling it to reverse-engineer the problem planning from the generated content. 
%     \item We then direct the LLM to generate relevant algorithms for the given problem and provide instructional tutorials to enable the agent reflecting on the underlying algorithms that related, and generate examples that are algorithmically close too.         
% \end{itemize}

% Additionally, we specify that the LLM should output the response in XML format for easy parsing of each example.

% from the acquired knowledge from the extensive training.

% The Self-retrieval Agent collects $k$ simiInstead of manually crafting similar examples, we instruct the Large Language Model (LLM) to retrieve problems from the acquired knowledge from the extensive training.
% The main motivation behind using Retrieval Augmented Generation (RAG) \cite{lewis2020retrieval} \eunus{didn't define?} \ashraful{updated} is to provide updated and analogous information to the model so that the model can get updated information to solve the current problem. Assuming no major changes in programming languages and problem solving algorithms, we can use self-retrieval here \eunus{not clear..}. 

% This retrieval agent employs the prompt depicted in Figure \ref{fig:prompt-agent-1}. The sequence of generation is crucial. Initially, we guide the LLM in generating similar and distinct problem with its solution, allowing it to subsequently reverse-engineer the planning of the problem from the generated content. We also instruct the LLM to produce algorithms relevant to the given problem and provide an instructive tutorial. Additionally, we specify that the LLM should generate the response in XML format for easy parsing of each example.

% While sharing similarities with Analogical Prompting \cite{yasunaga2023large}, our approach diverges in its multi-agent structure. Analogical Prompting combines exemplars generation and code generation into a single step, while our approach distributes tasks across different agents, enhancing the effectiveness of LLM prompting. Using a single step for generating exemplars and code may misguide the model during code generation. Results\ref{sec:results} also suggests that using multi-agent can improve the accuracy.

% \begin{figure*}
%     \centering
%     % \hspace*{-0.5cm}
%     \includegraphics[width=\textwidth]{figures/steps/step-2-prompt.pdf}
%     \caption{Prompt for Planning Agent. The example problem mentioned in this figure will come from the Self-retrieval Agent.}
%     % \rizwan{Need to mention the exemplars comes from the self-retrieval agent in caption here.}}
%     \label{fig:prompt-agent-2}
% \end{figure*}

\subsection{Planning Agent}
\label{subsec:our-algo-agent-2}

The second agent, the \emph{Planning Agent}, aims to create a step-by-step plan for the original problem. 
% While we could directly instruct an LLM model to do this or skip planning by using self-retrieved examples for code generation, this overlooks an important human step demonstrated in CoT \cite{CoT}: breaking down complex problems. 
Our \emph{Planning Agent} uses examples and their plans obtained from the retrieval agent to generate plans for the original problem. 
An straightforward approach would be to utilize all examples collectively to generate a single target plan. However, not all retrieved examples hold equal utility. Concatenating examples in a random order may compromise the LLM's ability to generate accurate planning. For instance, \citet{xu2023rereading} demonstrated that placing more relevant information (e.g., query) towards the end of the in-context input aids LLM reasoning more effectively than including relatively less relevant contexts. Therefore, we generate a distinct target plan for each retrieved example. Additionally, multiple plans offer diverse pathways to success. 

To help the generation steps in the following agents w/ the utility information for each  plan, our  designed prompt for planning agent asks the LLM to generate both plan, and a model confidence score. The prompt for this agent is shown in Figure \ref{fig:prompt-agent-2-short}. 
  

% We take the model confidence on how good the plan is to solve the original problem as the reward/utility score for the corresponding plan when designing the dynamic agent traversal scheme, discussed in \ref{sec:agent-traverse}. 


% Rereading, infact necesiates a scoreing, and the traversal schema.  
% Then we prompt the LLM to provide a confidence level regarding the problem's solvability using the generated planning.
% The motivation for processing each example separately, rather than collectively, is to prevent potential confusion for the LLM when exposed to multiple diverse examples, thereby ensuring the generation of accurate planning. The prompt for this agent is shown in Figure \ref{fig:prompt-agent-2}.

\begin{figure}
    \centering
    \hspace*{-0.3cm}
    \includegraphics[width=0.49\textwidth]{figures/steps/step-2-short.pdf}
    \vspace{-8mm}
    \caption{Prompt for \emph{Planning Agent}.} 
    % The example problem mentioned in this figure will come from the Self-retrieval Agent.}
    \label{fig:prompt-agent-2-short}
    \vspace{-4mm}
\end{figure}

\subsection{Coding Agent}
\label{subsec:our-algo-agent-3}
Next is the inevitable \emph{Coding Agent}. It takes the problem description, and a plan from the planning agent as input and translates the corresponding planning into code to solve the problem. During the traversing of agents, \emph{Coding Agent} takes the original problem and one particular plan from the \emph{Planning Agent}, generates the code, and test on sample IO.  
% The confidence level generated by the Planning Agent is used to sort the planning. 
If the initial code fails, the agent transfers it to the next agent for debugging. Otherwise, predicts that as the final solution.
% The prompt for this step is shown in Figure \ref{fig:prompt-agent-3}. 

\subsection{Debugging Agent}
\label{subsec:our-algo-agent-4}
The Debugging Agent leverages sample IO from the problem description to provide feedback on the correctness of the generated output. If the initial code fails in the sample IO, the LLM has the opportunity to modify its code iteratively, improving code quality for passing all test cases. This process is repeated $t$ times, generating modified planning and improved code for the problem. The prompt for this step is illustrated in Figure \ref{fig:prompt-agent-4-short}.

This agent is different from Reflexion \cite{shinn2023reflexion}, and AlphaCodium \cite{ridnik2024code} because they have generated additional test cases for evaluating the generated code, but our agent uses only the sample IO without generating test cases. The generated test cases may be a bottleneck because test case generation for complex problems is very hard. 
%We also found that in some cases Reflexion fails because of this step. 


We have shown the details prompts of each agent in Appendix \ref{app:prompts}.

\begin{figure}[h]
    \centering
    \hspace*{-0.3cm}
    \includegraphics[width=0.49\textwidth]{figures/steps/step-4-short.pdf}
    \vspace{-8mm}
    \caption{Prompt for \emph{Debugging Agent}.}
    \label{fig:prompt-agent-4-short}
    \vspace{-3mm}
\end{figure} 

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/qualitative-example.pdf}
    \caption{An example problem and solutions generated using Direct, CoT, Reflexion, and \tool prompting. \rizwan{mark sample I/O in the pic. This is not enough, we need to why, how? e.g., planner helps/wrong test case}}
    \label{fig:qualitative-example}
\end{figure*}  

\subsection{Dynamic Agent Traversal}
\label{sec:agent-traverse}
The dynamic traversal process starts with the Planning Agent, which generates plans along with their confidence scores. These plans are then sorted based on their confidence scores, with the highest-scoring plan forwarded to the Coding Agent. Subsequently, the Coding Agent translates the plan into code, which is then tested using the sample IOs. The code is returned for final evaluation if all sample IOs pass. However, if any IO fails, the code is passed to the Debugging Agent. The Debugging Agent attempts to rectify the code by analyzing the test report derived from the sample IO, highlighting the failure points. This debugging process is iterated up to $t$ times. It is returned if the Debugging Agent successfully resolves the issues and produces code that passes all sample IOs. %^for final evaluation\eunus{what is final evaluation here! we are returning the code??}. 
Otherwise, after $t$ iterations, the responsibility shifts back to the Planning Agent, which selects the plan with the next highest confidence score. Similar way, this iterative process continues for $k$ iterations, as there are $k$ plans from $k$ distinct example problems. This dynamic traversal of agents mimics the problem-solving approach of a programmer, who formulates plans, generates code, tests it, and iterates as needed. Consequently, our algorithm exhibits an $O(kt)$ complexity. One example of how \tool solves a problem compared to the Direct, Chain-of-thought \cite{wei2022chain}, and Reflexion \cite{shinn2023reflexion} approach is shown in Figure \ref{fig:qualitative-example}. The pseudo-code of our prompting approach is given in Algorithm \ref{alg:mapcoder}.



% \begin{figure*}
%     \centering
%     % \hspace*{-0.3cm}
%     \includegraphics[width=\textwidth]{figures/steps/step-3-prompt.pdf}
%     \caption{Prompt for Coding and Debugging Agent.}
%     \label{fig:prompt-agent-3}
% \end{figure*} 



==> sections/old/results-old.tex <==
\section{Results}
\label{sec:results}

We categorize datasets into two groups: easy problems and contest-level difficult problems. The easy problems category includes HumanEval \cite{chen2021codex}, HumanEval-ET \cite{dong2023codescore}, MBPP \cite{austin2021program}, and MBPP-ET \cite{dong2023codescore}. In contrast, the hard problems category comprises APPS \cite{hendrycks2021measuring}, CodeContests \cite{li2022competition}, and xCodeEval \cite{khan2023xcodeeval}. The results of these two categories are shown below:

\subsection{Results on Easy Datasets}
For the easy dataset category, we present the results of various prompting methods including Direct prompting, Chain of Thought Prompting (CoT) \cite{wei2022chain}, Self-planning prompting \cite{jiang2023self}, Analogical Reasoning prompting \cite{yasunaga2023large}, Reflexion \cite{shinn2023reflexion}, and our proposed approach, \ourapproach. The results, detailed in Table \ref{tab:easy-chatgpt-gpt4}, highlight the superiority of \ourapproach \space over other prompting methods. While Direct, CoT, Self-Planning, and Analogical Reasoning methods exhibit subtle bugs that could potentially be fixed through sample input-output testing, their lack of test case evaluation hinders their performance on several problems compared to our approach. Reflexion performs well due to its inclusion of test case evaluation and subsequent code modification based on the test report. However, our evaluation on ChatGPT for Reflexion reveals failure in eight cases in HumanEval and fifteen cases in MBPP due to erroneous test case generation. This proves that test case generation is not a trivail task and depends on the programming language, dataset, and model's capabilities \cite{chen2022codet}. Hence, we avoid generating new test cases and rely solely on sample input-output testing. Notably, in MBPP where sample test cases are unavailable, we skip debugging agent. We configure our model with $k=3$ and $t=5$ for HumanEval and HumanEval-ET, and $k=7$ and $t=0$ for MBPP and MBPP-ET.

\begin{table}[ht]
\centering
% \small
    \resizebox{\linewidth}{!}{
\begin{tabular}{c|l|c|c|c|c}
\hline
LLM & Approach & HE & HET & MP & MPT \\ \hline \hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{ChatGPT}} & Direct & \violetcell 48.1 & \violetcell 37.2 & \violetcell 49.8 & \violetcell 37.7 \\ \cline{2-6}
 & CoT & \violetcell 53.9 & \violetcell 45.5 & \violetcell 54.5 & \violetcell 39.6 \\  \cline{2-6}
 & Self-Planning & \violetcell  60.3 & \violetcell 46.2 & \violetcell 55.7 & \violetcell 41.9 \\  \cline{2-6}
 & Analogical & 63.4 & 57.9 & 70.3 & 46.6 \\  \cline{2-6}
 & Reflexion & 67.1 & 57.9 & 71.8 & 47.4 \\  \cline{2-6}
 & MapCoder & \greencell \bf 80.5 & \greencell \bf  70.1 & \greencell \bf  76.3 & \greencell \bf  51.6 \\ \hline \hline 
\multirow{6}{*}{\rotatebox[origin=c]{90}{GPT4}} & Direct & \cyancell 80.1 & 73.8 & \cyancell 80.1 & 54.2 \\  \cline{2-6}
 & CoT & 89.0 & 61.6 & 80.9 & 56.2 \\ \cline{2-6}
 & Self-Planning & 85.4 & 62.2 & 80.1 & 50.1 \\  \cline{2-6}
 & Analogical & 66.5 & 48.8 & 57.2 & 34.3 \\  \cline{2-6}
 & Reflexion & \cyancell 91.0 & 78.7 & \cyancell 77.1 & 51.6 \\  \cline{2-6}
 & MapCoder & \greencell {\bf 93.9} & & &\\ \hline 
\end{tabular}
}
\caption{Performance of different prompting approach on HumanEval (HE), HumanEval-ET (HET), MBPP (MP), and MBPP-ET (MPT). \rizwan{put a cap on methods for which you have reported numbers from diff papers and cite that paper in caption. For example, check Table 2 in https://arxiv.org/pdf/2401.05787.pdf. Also add a row of previous sota or mark them with symbol in the curremt table.}}
\label{tab:easy-chatgpt-gpt4}
\end{table}


